Analyzing and Improving Greedy 2-Coordinate Updates for Equality-Constrained Optimization via Steepest Descent in the 1-Norm

We consider minimizing a smooth function subject to a summation constraint over its variables. By exploiting a connection between the greedy 2-coordinate update for this problem and equality-constrained steepest descent in the 1-norm, we give a convergence rate for greedy selection under a proximal Polyak-Lojasiewicz assumption that is faster than random selection and independent of the problem dimension $n$. We then consider minimizing with both a summation constraint and bound constraints, as arises in the support vector machine dual problem. Existing greedy rules for this setting either guarantee trivial progress only or require $O(n^2)$ time to compute. We show that bound- and summation-constrained steepest descent in the L1-norm guarantees more progress per iteration than previous rules and can be computed in only $O(n \log n)$ time.

==> Content/algorithm-GS1.tex <==
\begin{algorithm}
\caption{GS-1}\label{alg:euclid}
\begin{algorithmic}[1]
\Function{GS-1}{$x,f,L,l,u$}
\State $x_{0} \gets 0; x_{n+1} \gets 0; i \gets 1; j \gets n; d \gets 0;$
\While 1
\State $\delta \gets \frac{1}{4L} \left(\nabla_i f(x) - \nabla_j f(x) \right)$
\State $\omega = \sum\limits_{p=0}^{i-1} x_p-l_p$; $\kappa  = \sum\limits_{q=j+1}^{n+1} u-x_q$
\If{$\delta- \omega  < 0\And 
\delta - \kappa < 0$}
    \If {$\omega < \kappa$} $d_i = \omega  - \kappa$ ; break;
    \Else \hspace{0.1cm}$d_j =\omega  - \kappa$; break;
    \EndIf
\ElsIf {$\delta- \omega  < 0$} $d_j = \omega  - \kappa$; break;
\ElsIf {$\delta- \kappa < 0$} $d_i = \omega  - \kappa$; break;
\EndIf
\If{$x_i +\omega -\delta \geq l_i \And x_j - \kappa+\delta \leq u_j$}
    \State $d_i = \omega -\delta ; d_j = \delta-\kappa$; break;
\EndIf
\If{$x_i +\omega -\delta < l_i \And x_j - \kappa+\delta > u_j$}
    \If{$l_i - (x_i +\omega -\delta) > x_j - \kappa+\delta- u_j$}
    \State $d_i = l- x_i$; $i\gets i+1$
    \Else
    \State $d_j = u- x_j$; $j\gets j-1$
    \EndIf
\ElsIf{$x_i+\omega  - \delta< l_i$} $d_i=l-x_i$; $i\gets i+1$
\Else \hspace{0.1cm}$d_j = u- x_j$; $j\gets j-1$
\EndIf
\EndWhile\label{euclidendwhile}
\State \textbf{return} $d$
\EndFunction
\end{algorithmic}
\end{algorithm}

==> Content/notations.tex <==
We call the indices of a parameter vector $x \in \mathbb{R}^n$, \textit{coordinates}. The notation $d_{ij} \in \mathbb{R}^{2}$ denotes the elements of the vector $d$ corresponding to the block of coordinates $i,j$ and we use $B$ to indicate the set of coordinate blocks considered by the algorithm. $\nabla_{ij} f(x) \in \mathbb{R}^2$ denotes the gradient of the block.
\begin{definition}[Support of a Vector]
    The support of a vector $d \in \R^n$ is the maximal set of indices $\mathcal{I} \subseteq \{1,\dots,n\}$ satisfying $d_i \neq 0 \textup{ for } i \in \mathcal{I}.$
    We indicate the support of $d$ by $\supp(x)$. \\
\end{definition}

\begin{definition}[Conformal Vectors]
Let $d, d' \in \R^n$. We say the vector $d'$ is conformal to $d$ if
\[ \supp(d') \subseteq \supp(d) \quad \textup{and} \quad d_i d_i' \geq 0 \quad \textup{for } i = 1 \dots n.  \]
\end{definition}

\begin{definition}[Elementary Vectors]
Let $S$ be a subspace of $\R^n$. A vector $d \in S$ is called an elementary vector of $S$ if
\begin{align*}
\nexists d' \in S, d' \neq 0 &\mbox{\textup{ such that}} \\
\mbox{\textup{$d'$ is conformal to $d$ and} } &\supp(d') \neq \supp(d).
\end{align*}
\end{definition}

==> Content/valueAddedOld.tex <==

For some problems where we have a simple equality constraint, we also have lower and/or upper bounds on the values of the individual variables. This results in a problem of the form
\[
\min_{x\in\R^n} f(x), \hspace{0.3 cm}\text{subject to     } \sum\limits_{i=1}^n x_i =\gamma, l_i \leq x_i \leq u_i.
\]
This framework includes our motivating problems of optimizing over the probability simplex, or optimizing SVMs with an unregularized bias. A natural extension of the greedy rule~\eqref{eq:ik} to this problem is~\citep[see][]{beck20142}
\[
i_k \in \argmax_{i \;|\; x_i^k > l_i}\nabla_i f(x^k), \quad j_k \in \argmin_{j \; | \; x_j^k < u_i}\nabla_j f(x^k),
\]
which is the rule used in (for example) the first versions of LIBSVM. \red{Hmmm, I guess this is the GS-s rule and we should focus on GS-q since the course project result does not apply to GS-s and I think they have the same cost.}
With bound constraints we use a $d^k$ of form~\eqref{eq:dk} but where $\delta^k$ is defined so that the step respects the constraints,
\[
\delta^k = \min\left\{\frac{1}{2L_2}(\nabla_{i_k}f(x^k) - \nabla_{j_k}f(x^k)),x_i^k - l_i, u_i - x_i^k\right\}.
\]
Note that if the variables are unbounded (all $l_i = -\infty$ and all $u_i=\infty$) then we obtain the equality-constrained algorithm. However, the bound-constrained greedy coordinate descent algorithm does not in general correspond to performing steepest descent in the 1-norm. This makes the bound constrained setting more difficult to analyze. In this section we give three approaches to addressing the bound constrained case: a dimension-dependent analysis of the greedy method, a dimension-independent analysis requiring a modified algorithm, and finally a hybrid analysis of the basic greedy method that only has a dimension dependence on the initial iterations.

\subsection{Analysis using conformal realizations}
Here, we show linear convergence of the greedy 2-coordinate descent under a linear equality constraint and bound constraint for the problem in \eqref{eq:box}. Lemma \ref{lemma:non_elementary_realizations} is the key property we use in this approach.
\begin{lemma}[Conformal Realizations]
    \label{lemma:non_elementary_realizations}
    Let $S$ be a subspace of $\R^n$ and $t = \min_{x \in S} \supp(x)$.
    Let $\tau \in \{t, \dots, n\}$. Then every non-zero vector $x$ of $S \subseteq \R^n$ can be realized as the sum
    \[ x = d_1 + \dots + d_{s} + d_{s+1}, \]
    where $d_1, \dots, d_{s}$ are elementary vectors of $S$ that are conformal to $x$ and $d_{s+1} \in S$ is a vector conformal to $x$ with $\supp(d_{s+1}) = \tau$.  Furthermore, $s \leq n - \tau$. 
\end{lemma}
See Appendix \ref{appendix:conformal_realizations} for proof. Lemma \ref{lemma:non_elementary_realizations} was first established by \citet[Proposition~6.1]{tseng2009block} as part of a larger result. We rediscovered it independently and include our proof for completeness. 

We introduce some more definitions needed to derive convergence. We denote the maximum of the block-coordinate Lipschitz constants by
\[ L_{max} = \max_{b_i \in B} L_{b_i} \]
Let $H \in \R^{n \times n}$ be a positive semi-definite curvature matrix.
The principal sub-matrix corresponding to block $b_i \in B$ is  $H_{b_i}$; the norm induced by the positive semi-definite sub-matrix is 
\[ \norm{x_{b_i}}_{H_{b_i}} = \sqrt{x_{b_i}^\top H_{b_i} x_{b_i}}. \] 
If $H$ satisfies the generalized inequality $H_{b_i} \preceq L_{b_i} \vI$ for all $b_i \in B$, then the norm inequality
\begin{align}
\norm{x_{b_i}}_{H_{b_i}}^2 \leq L_{b_i} \norm{x_{b'_i}}_2^2 \leq L_{max} \norm{x_{b_i}}_2^2, \label{eq:principle_submatrix_norms}
\end{align}
holds for all blocks $b_i \in B$. Now, Theorem \ref{theorem:convergence_box} below derives the convergence rate.
\begin{theorem}
\label{theorem:convergence_box}
Let the function $F(x)= f(x)+ h(x)$, where $f: \mathbb{R}^n \xrightarrow{}  \mathbb{R}$ is a smooth function and $h(x)$ is the box constraint indicator, 
\begin{align*}
    h(x) =  \begin{cases}
        0 & \mbox{if $0 \leq  x_i \leq C$ for all $i \in \{1, \dots, n\}$}\\
        \infty & \mbox{otherwise}
        \end{cases}
\end{align*}
satisfies prox-PL condition with constant $\mu$. Assume $f$ has block-wise Lipschitz continuous gradients and let $L_{max}= \max_{b_i \in B} L_{b_i}$. Assume that the matrices $\{H^k\}$ satisfy $\nabla^2 f(x^k) \preceq H^k \preceq L_{max} \vI$ at every iteration $k$. Solving the problem
\begin{align}
   &\min_{x\in\R^n} F(x), \nonumber \hspace{0.3 cm}\\\text{subject to     } & A^T x =\gamma.
\end{align}
with 2-coordinate descent with coordinate blocks selected according to the GS-q rule obtains the following linear rate of convergence:
  \begin{equation}
    F(x^k) - F^* \leq \parens{1 - \frac{\mu}{L_{max}(n - 1)}}^k \parens{F(x^0) - F^*}. 
  \end{equation} 
  

\end{theorem}
We provide the proof in Appendix \ref{proof:convergence_box}. Unlike our convergence rate in the case with only linear equality constraint, this rate is dependent on problem dimension $n$. However, this rate is still faster than that of randomized selection \eqref{eq:random} which is dependent on $n^2$.
% Show the $(1-\mu/L(n-1)$ result. Say that unfortunately is dimension dependent, but still faster than random.


\subsection{Analysis using steepest descent in the 1-norm}

One of the first approaches we explored is to extend the analysis in  Theorem \ref{result}, using the connection to steepest descent in the $1$-norm, to include the bound constraint. This approach could provide same convergence rate as \eqref{eq:GSqRate}. However, with bound constraints, Lemma \eqref{lemma:sd} is no longer applicable; that is, steepest descent could update more than $2$ coordinates in every iteration in order to satisfy both the constraints. Intuitively, if after the update the parameter $x$ goes out of bound, one way to handle it is to project it back into the feasible set. This projection step may violate the equality constraint and the algorithm will need to update more coordinates in order to satisfy the constraints. Also, it is not immediately obvious how to compute these coordinates efficiently.  
%  This is because with bound constraints and an equality constraint the steepest descent direction in the 1-norm may update more than two coordinates.

% We could do steepest descent in L1-norm and get the same result, $(1-\mu_1/L)$. But, this might involve updating multiple coordinates. And it is not obvious how to compute the L1-norm steepest descent efficiently.

\subsection{Analysis using good and bad steps}
One thing we observed is, when the update is within the feasible region, the bound given in \eqref{result} is applicable. We explored this approach by categorizing the updates into good and bad steps, like in the work \cite{karimireddy2019efficient}. In any iteration $k$, if $l_i \leq x_i^k - d_i^k \leq u_i $ and $l_i \leq x_j^k + d_j^k \leq u_i $, we call it a \textbf{good step}. When the update goes out of bounds, we call it a \textbf{bad step}. That is, if $l_i < x_i^k < u_i$ and $l_i < x_j^k < u_i$, but $x_i^k - d_i^k < l_i $ and/or $x_j^k + d_j^k > u_i $, we call it a bad step. Now, showing faster convergence involves either deriving a faster rate for the bad steps or bounding the number of bad steps the algorithm can take.

The work \cite{karimireddy2019efficient} approach this problem bound the number of bad steps. They argue that at most half steps are bad steps, as the greedy coordinate descent algorithm guarantees to take a good step after a bad step while updating single coordinate in every iteration. However, this argument is not applicable in our setting, as with equality constraints, we update atleast $2$ coordinates, if a variable is picked again it could still take a bad step even though it moves away from bound. We could make a combinatorial argument that the number of bad steps is bounded as in ~\citet[][Theorem~8]{lacoste2015global}, but the resulting bound could be much looser.



% \citet{karimireddy2019efficient} use good steps and bad steps and cross steps for bound constraints. Argue that at most half steps are bad steps, because after a bad step you must take a good step with that variable. Unfortunately, this does not work with equality constraints, since if you pick a variable again it might still take a bad step even though it moves away from bound. Could make a combinatorial argument that the number of bad steps is bounded as in~\citet[][Theorem~8]{lacoste2015global}, but bound is loose because it has factorials (worse than random?).

There are good steps where L1-norm steepest descent = q-GCD, and bad steps where get the course project rate. Without equality constraint, you take bad steps only half the time. Counter-example that this does not work for equality constraints? But asymptotically, you only take good steps. 

Active-set identification: show that after some 'k' iterations you only do good steps. Active set complexity: give bounds on 'k'.

\subsection{Active-Set Identifying Steps}

Nutini et al. consider active-set complexity for GCD with no equality. But they have this bad dependence on ``variable closest to boundary''. We could take ``very bad steps'' half the time (when possible), where we choose one (or both) coorindates as those very close to boundary. Gets rid of this dependence at the cost of doubling active set complexity. (Works for equality and non-equality case.)



